Nudging Beyond the Comfort Zone: Efficient Strategy-Guided Exploration for RLVR

Reinforcement learning with verifiable rewards (RLVR) is a scalable paradigm for improving the mathematical reasoning of large language models, but it is fundamentally limited by exploration: the policy can only improve on trajectories it has already sampled. Sampling more rollouts alleviates this at prohibitive compute cost, while objective-level modifications offer little control over what is explored. We propose NudgeRL, a framework for structured, diversity-driven exploration in RLVR whose core component, Strategy Nudging, conditions each rollout on a lightweight strategy-level context, without requiring the context generator to solve the problem itself. To learn from such exploration, we decompose the advantage into inter- and intra-context terms and add a policy correction term that transfers discovered behaviors back to the base policy. Across five mathematical reasoning benchmarks, NudgeRL with 8 rollouts matches the strongest GRPO baseline using 32 rollouts with roughly 5 times fewer total tokens and 2.9 times less training compute. Our code is available at https://github.com/tally0818/NudgeRL.

==> text/prompts/nudge_sol.tex <==
\begin{promptbox}{NudgeRL Solution}
    \texttt{<start\_working\_out>}

    We are given a right triangle $\triangle ABC$ with $\angle A = 90^\circ$ and hypotenuse $BC = 38$. There are two points $K$ and $L$ inside the triangle such that:
    \[
    AK = AL = BK = CL = KL = 14
    \]

    We are to find the area of quadrilateral $BKLC$, which is expressed as $n\sqrt{3}$, and find $n$.

    ---

    \#\#\# Step 1: Understand the configuration

    We have:
    - $\angle A = 90^\circ$, so $AB$ and $AC$ are legs, $BC = 38$ is the hypotenuse.
    - Points $K$ and $L$ are inside the triangle.
    - All of the following distances are equal to 14:
      - $AK = AL = BK = CL = KL = 14$

    This suggests symmetry. Since $AK = AL$, and $BK = CL$, and $KL = 14$, it's likely that $K$ and $L$ are symmetric with respect to the angle bisector or the median from $A$.

    Moreover, $AK = AL$ suggests that $K$ and $L$ lie on the perpendicular bisector of $BL$ or something symmetric.

    But let's try to exploit symmetry.

    ---

    \#\#\# Step 2: Consider symmetry

    Since $AK = AL$ and $BK = CL$, and the triangle is right-angled at $A$, a natural symmetry is about the angle bisector of $\angle A$, which in a right triangle is the line $y = x$ if we place $A$ at the origin and $AB$, $AC$ along the axes.

    Let's place the triangle in coordinate plane:

    Let:
    - $A = (0, 0)$
    - $B = (b, 0)$
    - $C = (0, c)$

    Then $BC = 38$, so by Pythagoras:
    \[
    b^2 + c^2 = 38^2 = 1444
    \]

    We are to find points $K$ and $L$ such that:
    - $AK = AL = 14$
    - $BK = 14$
    - $CL = 14$
    - $KL = 14$

    Let's suppose that due to symmetry, $K$ and $L$ are symmetric with respect to the line $y = x$. Then:

    Let $K = (x, y)$, then $L = (y, x)$

    Then:
    - $AK = \sqrt{x^2 + y^2} = 14 \Rightarrow x^2 + y^2 = 196$ --- (1)
    - $BK = \sqrt{(x - b)^2 + y^2} = 14 \Rightarrow (x - b)^2 + y^2 = 196$ --- (2)
    - $CL = \sqrt{(y - c)^2 + x^2} = 14 \Rightarrow (y - c)^2 + x^2 = 196$ --- (3)
    - $KL = \sqrt{(x - y)^2 + (y - x)^2} = \sqrt{2(x - y)^2} = \sqrt{2} |x - y| = 14$

    So:
    \[
    \sqrt{2} |x - y| = 14
    \Rightarrow
    |x - y| = \frac{14}{\sqrt{2}} = 7\sqrt{2}
    \]

    So $x - y = \pm 7\sqrt{2}$. Without loss of generality, assume $x > y$, so $x - y = 7\sqrt{2}$ --- (4)

    ---

    \#\#\# Step 3: Use equations (1), (2), (3), (4)

    From (1): $x^2 + y^2 = 196$

    From (4): $x = y + 7\sqrt{2}$

    Plug into (1):

    \[
    \begin{aligned}
    (y + 7\sqrt{2})^2 + y^2 &= 196 \\
    y^2 + 14\sqrt{2}y + 98 + y^2 &= 196 \\
    2y^2 + 14\sqrt{2}y + 98 &= 196 \\
    2y^2 + 14\sqrt{2}y &= 98 \\
    y^2 + 7\sqrt{2}y &= 49
    \end{aligned}
    \]

    This is a quadratic in $y$. Let's solve it.

    Complete the square:

    \[
    \begin{aligned}
    y^2 + 7\sqrt{2}y &= 49 \\
    y^2 + 7\sqrt{2}y + \left( \frac{7\sqrt{2}}{2} \right)^2
    &=
    49 + \left( \frac{7\sqrt{2}}{2} \right)^2 \\
    y^2 + 7\sqrt{2}y + \frac{49 \cdot 2}{4}
    &=
    49 + \frac{98}{4}
    =
    49 + 24.5
    =
    73.5
    \end{aligned}
    \]

    So:
    \[
    \left( y + \frac{7\sqrt{2}}{2} \right)^2 = 73.5 = \frac{147}{2}
    \]

    So:
    \[
    y = -\frac{7\sqrt{2}}{2} \pm \sqrt{\frac{147}{2}}
    \]

    This is messy, and we haven't yet used the other conditions involving $b$ and $c$. So perhaps we should go back to equations (2) and (3).
\end{promptbox}
\begin{promptbox}{NudgeRL Solution (Cont.)}
    ---

    From equation (2): $(x - b)^2 + y^2 = 196$

    From (1): $x^2 + y^2 = 196$

    Subtract (1) - (2):

    \[
    \begin{aligned}
    (x^2 + y^2) - [(x - b)^2 + y^2] &= 0 \\
    x^2 - (x^2 - 2bx + b^2) &= 0 \\
    x^2 - x^2 + 2bx - b^2 &= 0 \\
    2bx &= b^2
    \end{aligned}
    \]

    So $b = 2x$

    Similarly, go to equation (3): $(y - c)^2 + x^2 = 196$

    From (1): $x^2 + y^2 = 196$

    Subtract (3) - (1):

    \[
    \begin{aligned}
    [(y - c)^2 + x^2] - [x^2 + y^2] &= 0 \\
    (y - c)^2 - y^2 &= 0 \\
    y^2 - 2cy + c^2 - y^2 &= 0 \\
    -2cy + c^2 &= 0
    \end{aligned}
    \]

    So $c = 2y$

    Now we have:
    - $b = 2x$
    - $c = 2y$
    - $x^2 + y^2 = 196$
    - $x - y = 7\sqrt{2}$

    And also from the hypotenuse:
    \[
    \begin{aligned}
    b^2 + c^2 &= 1444 \\
    (2x)^2 + (2y)^2 &= 1444 \\
    4x^2 + 4y^2 &= 1444 \\
    x^2 + y^2 &= 361
    \end{aligned}
    \]

    Wait! This contradicts equation (1), which said $x^2 + y^2 = 196$.

    So contradiction!

    That means our assumption that $K = (x, y)$, $L = (y, x)$ is invalid?

    But why? Because $AK = AL = 14$, and symmetry about $y = x$ makes sense, but the distance from $K$ to $B$ and $L$ to $C$ may not match unless the legs are in a certain ratio.

    But we get a contradiction: $x^2 + y^2 = 196$ from $AK = 14$, but from $b^2 + c^2 = 1444$, we get $x^2 + y^2 = 361$, which is not equal.

    So our assumption must be wrong.

    Where did we go wrong?

    Ah --- in the step where we said from (2) and (1), we got $b = 2x$. Let's double-check:

    From (1): $x^2 + y^2 = 196$

    From (2): $(x - b)^2 + y^2 = 196$

    Subtract (1) from (2):

    \[
    \begin{aligned}
    (x - b)^2 - x^2 &= 0 \\
    x^2 - 2bx + b^2 - x^2 &= 0 \\
    -2bx + b^2 &= 0 \\
    b(b - 2x) &= 0
    \end{aligned}
    \]

    So either $b = 0$ (impossible) or $b = 2x$

    Same for $c = 2y$

    So the algebra seems correct.

    But then $b^2 + c^2 = 4x^2 + 4y^2 = 4(x^2 + y^2) = 4 \times 196 = 784$

    But we are told $BC = 38$, so $b^2 + c^2 = 38^2 = 1444$

    But $784 \ne 1444$

    Contradiction.

    So our assumption that $K$ and $L$ are symmetric across $y = x$ must be invalid.

    Alternative idea: Maybe $K$ and $L$ are symmetric with respect to the altitude from $A$, or the angle bisector?

    Alternatively, perhaps the configuration is such that $K$ and $L$ are located so that they are equidistant from $A$, $B$, $C$, and each other.

    Wait --- we are given:

    - $AK = AL = 14$
    - $BK = 14$
    - $CL = 14$
    - $KL = 14$

    So:
    - $K$ is at distance 14 from $A$ and $B$
    - $L$ is at distance 14 from $A$ and $C$
    - $K$ and $L$ are at distance 14 from each other
\end{promptbox}
\begin{promptbox}{NudgeRL Solution (Cont.)}
    So $K$ lies at intersection of circles:
    - Circle centered at $A$ with radius 14
    - Circle centered at $B$ with radius 14

    Similarly, $L$ lies at intersection of:
    - Circle centered at $A$ with radius 14
    - Circle centered at $C$ with radius 14

    So both $K$ and $L$ are at intersection of circle $A$ and circle $B$, and $A$ and $C$ respectively.

    So we can find coordinates.

    ---

    \#\#\# Step 4: Coordinate geometry setup

    Let's place:
    - $A = (0, 0)$
    - $B = (b, 0)$
    - $C = (0, c)$

    Then $b^2 + c^2 = 38^2 = 1444$

    Now, find intersection of circle centered at $A(0,0)$ with radius 14 and circle centered at $B(b,0)$ with radius 14.

    Equation of circle at $A$: $x^2 + y^2 = 196$

    Equation of circle at $B$: $(x - b)^2 + y^2 = 196$

    Subtract:

    \[
    \begin{aligned}
    (x - b)^2 - x^2 &= 0 \\
    x^2 - 2bx + b^2 - x^2 &= 0 \\
    -2bx + b^2 &= 0 \\
    x &= \frac{b}{2}
    \end{aligned}
    \]

    Plug into $x^2 + y^2 = 196$:

    \[
    \begin{aligned}
    \left(\frac{b}{2}\right)^2 + y^2 &= 196 \\
    \frac{b^2}{4} + y^2 &= 196 \\
    y^2 &= 196 - \frac{b^2}{4}
    \end{aligned}
    \]

    So $y = \pm \sqrt{196 - \frac{b^2}{4}}$

    Since $K$ is inside the triangle, we take $y > 0$, so
    \[
    y_K = \sqrt{196 - \frac{b^2}{4}}
    \]

    Similarly, find $L$: intersection of circle at $A$ and circle at $C(0,c)$

    Circle at $C$: $x^2 + (y - c)^2 = 196$

    Subtract from $x^2 + y^2 = 196$:

    \[
    \begin{aligned}
    x^2 + y^2 - [x^2 + (y - c)^2] &= 0 \\
    y^2 - (y^2 - 2cy + c^2) &= 0 \\
    2cy - c^2 &= 0 \\
    y &= \frac{c}{2}
    \end{aligned}
    \]

    Then:
    \[
    x^2 + \left(\frac{c}{2}\right)^2 = 196
    \Rightarrow
    x^2 = 196 - \frac{c^2}{4}
    \]

    So:
    \[
    x_L = \sqrt{196 - \frac{c^2}{4}}
    \]

    (positive, since inside triangle)

    So:
    - $K = \left( \frac{b}{2}, \sqrt{196 - \frac{b^2}{4}} \right)$
    - $L = \left( \sqrt{196 - \frac{c^2}{4}}, \frac{c}{2} \right)$

    We are given that $KL = 14$

    So compute distance between $K$ and $L$:

    \[
    KL^2 =
    \left( \frac{b}{2} - \sqrt{196 - \frac{c^2}{4}} \right)^2
    +
    \left( \sqrt{196 - \frac{b^2}{4}} - \frac{c}{2} \right)^2
    =
    14^2 = 196
    \]
\end{promptbox}
\begin{promptbox}{NudgeRL Solution (Cont.)}
    Let's define:
    - $p = \frac{b}{2}$
    - $q = \frac{c}{2}$

    Then $b = 2p$, $c = 2q$

    Then:
    \[
    b^2 + c^2 = 4p^2 + 4q^2 = 4(p^2 + q^2) = 1444
    \Rightarrow
    p^2 + q^2 = 361
    \]

    Now express the coordinates:
    - $K = (p, \sqrt{196 - p^2})$
    - $L = (\sqrt{196 - q^2}, q)$

    Then:
    \[
    KL^2 =
    (p - \sqrt{196 - q^2})^2
    +
    (\sqrt{196 - p^2} - q)^2
    =
    196
    \]

    Expand:

    First term:
    \[
    (p - \sqrt{196 - q^2})^2
    =
    p^2 - 2p\sqrt{196 - q^2} + (196 - q^2)
    \]

    Second term:
    \[
    (\sqrt{196 - p^2} - q)^2
    =
    (196 - p^2) - 2q\sqrt{196 - p^2} + q^2
    \]

    Add both:

    \[
    \begin{aligned}
    &p^2 + 196 - q^2 + 196 - p^2 + q^2 \\
    &\qquad - 2p\sqrt{196 - q^2} - 2q\sqrt{196 - p^2}
    =
    196
    \end{aligned}
    \]

    Simplify:

    - $p^2 - p^2 = 0$
    - $-q^2 + q^2 = 0$
    - $196 + 196 = 392$

    So:
    \[
    392 - 2p\sqrt{196 - q^2} - 2q\sqrt{196 - p^2} = 196
    \]

    Bring to left:

    \[
    \begin{aligned}
    392 - 196
    &=
    2p\sqrt{196 - q^2} + 2q\sqrt{196 - p^2} \\
    196
    &=
    2p\sqrt{196 - q^2} + 2q\sqrt{196 - p^2} \\
    98
    &=
    p\sqrt{196 - q^2} + q\sqrt{196 - p^2}
    \end{aligned}
    \]

    Now recall that $p^2 + q^2 = 361$

    Let's define $x = p$, $y = q$, so:
    - $x^2 + y^2 = 361$
    - $x\sqrt{196 - y^2} + y\sqrt{196 - x^2} = 98$

    Let's try to simplify or guess values.

    Note that $x^2 + y^2 = 361$, so $x^2, y^2 \le 361$

    Also:
    \[
    196 - x^2 \ge 0
    \Rightarrow
    x^2 \le 196
    \]
    similarly $y^2 \le 196$

    Let's suppose $x = y$. Then:
    \[
    2x^2 = 361
    \Rightarrow
    x^2 = 180.5
    \Rightarrow
    x \approx 13.43
    \]

    Check if the equation holds:

    Left side:
    \[
    x\sqrt{196 - x^2} + x\sqrt{196 - x^2}
    =
    2x\sqrt{196 - x^2}
    \]

    Since:
    \[
    x^2 = 180.5
    \Rightarrow
    196 - x^2 = 15.5
    \]

    We have:
    \[
    \sqrt{15.5} \approx 3.937
    \]

    and
    \[
    x \approx \sqrt{180.5} \approx 13.43
    \]

    So:
    \[
    2 \times 13.43 \times 3.937
    \approx
    2 \times 52.9
    \approx
    105.8 \ne 98
    \]

    Too big.

    So $x = y$ is too big.

    We need smaller value.

    Try to assume $x^2 = a$, $y^2 = 361 - a$

    We want:
    \[
    \sqrt{a} \sqrt{196 - (361 - a)}
    +
    \sqrt{361 - a} \sqrt{196 - a}
    =
    98
    \]

    Simplify:

    \[
    196 - (361 - a) = a - 165
    \]

    So:
    \[
    \sqrt{a(a - 165)}
    +
    \sqrt{(361 - a)(196 - a)}
    =
    98
    \]
\end{promptbox}
\begin{promptbox}{NudgeRL Solution (Cont.)}
    Now define function:
    \[
    f(a)
    =
    \sqrt{a(a - 165)}
    +
    \sqrt{(361 - a)(196 - a)}
    \]

    Domain:
    \[
    a > 165
    \]
    since:
    \[
    a(a - 165) \ge 0
    \]

    Also:
    \[
    a \le 196,
    \qquad
    361 - a \ge 0
    \Rightarrow
    a \le 361
    \]

    so:
    \[
    a \in (165, 196]
    \]

    Try $a = 169$:

    - $a(a - 165) = 169(4) = 676$, $\sqrt{676} = 26$
    - $361 - 169 = 192$
    - $196 - 169 = 27$
    - $192 \times 27 = 5184$
    - $\sqrt{5184} = 72$

    Sum:
    \[
    26 + 72 = 98
    \]

    Perfect!

    So:
    \[
    a = 169
    \]

    Hence:
    \[
    x^2 = 169
    \Rightarrow
    x = 13
    \]

    and:
    \[
    y^2 = 361 - 169 = 192
    \Rightarrow
    y = \sqrt{192} = 8\sqrt{3}
    \]

    Now check:
    \[
    x^2 + y^2 = 169 + 192 = 361
    \]

    Also:
    \[
    \sqrt{a(a - 165)}
    =
    \sqrt{169 \cdot 4}
    =
    \sqrt{676}
    =
    26
    \]

    and:
    \[
    \sqrt{(361 - 169)(196 - 169)}
    =
    \sqrt{192 \cdot 27}
    =
    \sqrt{5184}
    =
    72
    \]

    Sum:
    \[
    26 + 72 = 98
    \]

    Perfect.

    So:
    - $p = x = 13$
    - $q = y = \sqrt{192} = 8\sqrt{3}$

    Then:
    - $b = 2p = 26$
    - $c = 2q = 16\sqrt{3}$

    Check:
    \[
    b^2 + c^2
    =
    26^2 + (16\sqrt{3})^2
    =
    676 + 256 \cdot 3
    =
    676 + 768
    =
    1444
    =
    38^2
    \]

    Good.

    Now we have coordinates:
    \[
    K =
    \left(
    \frac{b}{2},
    \sqrt{196 - \left(\frac{b}{2}\right)^2}
    \right)
    =
    (13, \sqrt{196 - 169})
    =
    (13, \sqrt{27})
    =
    (13, 3\sqrt{3})
    \]

    and:
    \[
    L =
    \left(
    \sqrt{196 - \left(\frac{c}{2}\right)^2},
    \frac{c}{2}
    \right)
    \]

    Since:
    \[
    \frac{c}{2} = 8\sqrt{3}
    \]

    and:
    \[
    \left(\frac{c}{2}\right)^2 = (8\sqrt{3})^2 = 192
    \]

    So:
    \[
    \sqrt{196 - 192} = \sqrt{4} = 2
    \]

    Thus:
    \[
    L = (2, 8\sqrt{3})
    \]
\end{promptbox}
\begin{promptbox}{NudgeRL Solution (Cont.)}
    Therefore:
    - $K = (13, 3\sqrt{3})$
    - $L = (2, 8\sqrt{3})$

    Now we want the area of quadrilateral $BKLC$

    Points:
    - $B = (26, 0)$
    - $K = (13, 3\sqrt{3})$
    - $L = (2, 8\sqrt{3})$
    - $C = (0, 16\sqrt{3})$

    Quadrilateral $BKLC$ --- in order:
    \[
    B \to K \to L \to C \to B
    \]

    We can compute its area using shoelace formula.

    List the points in order:

    1. $B = (26, 0)$
    2. $K = (13, 3\sqrt{3})$
    3. $L = (2, 8\sqrt{3})$
    4. $C = (0, 16\sqrt{3})$

    Back to $B = (26, 0)$

    Shoelace formula:

    \[
    \text{Area}
    =
    \frac{1}{2}
    \left|
    \sum x_i y_{i+1}
    -
    \sum y_i x_{i+1}
    \right|
    \]

    Compute:
    \[
    \sum x_i y_{i+1}
    \]

    - $26 \cdot 3\sqrt{3} = 78\sqrt{3}$
    - $13 \cdot 8\sqrt{3} = 104\sqrt{3}$
    - $2 \cdot 16\sqrt{3} = 32\sqrt{3}$
    - $0 \cdot 0 = 0$

    Sum:
    \[
    (78 + 104 + 32)\sqrt{3}
    =
    214\sqrt{3}
    \]

    Compute:
    \[
    \sum y_i x_{i+1}
    \]

    - $0 \cdot 13 = 0$
    - $3\sqrt{3} \cdot 2 = 6\sqrt{3}$
    - $8\sqrt{3} \cdot 0 = 0$
    - $16\sqrt{3} \cdot 26 = 416\sqrt{3}$

    Sum:
    \[
    (0 + 6 + 0 + 416)\sqrt{3}
    =
    422\sqrt{3}
    \]

    Now:
    \[
    \text{Area}
    =
    \frac{1}{2}
    |214\sqrt{3} - 422\sqrt{3}|
    =
    \frac{1}{2} \cdot 208\sqrt{3}
    =
    104\sqrt{3}
    \]

    So:
    \[
    n = 104
    \]

    ---

    Final Answer:

    \texttt{<SOLUTION>}104\texttt{</SOLUTION>}
\end{promptbox}
